Simpler Hyperparameter Optimization for Software Analytics: Why, How, When?

How can we make software analytics simpler and faster? One method is to match the complexity of analysis to the intrinsic complexity of the data being explored. For example, hyperparameter optimizers find the control settings for data miners that improve the predictions generated via software analytics. Sometimes, very fast hyperparameter optimization can be achieved by "DODGE-ing"; i.e. simply steering way from settings that lead to similar conclusions. But when is it wise to use that simple approach and when must we use more complex (and much slower) optimizers?} To answer this, we applied hyperparameter optimization to 120 SE data sets that explored bad smell detection, predicting Github issue close time, bug report analysis, defect prediction, and dozens of other non-SE problems. We find that the simple DODGE works best for data sets with low "intrinsic dimensionality" (u ~ 3) and very poorly for higher-dimensional data (u > 8). Nearly all the SE data seen here was intrinsically low-dimensional, indicating that DODGE is applicable for many SE analytics tasks.

==> replies-v1.tex <==
 \setcounter{page}{0}
    \pagenumbering{arabic}
    
    \section*{Response to reviewers}
    
 \subsection*{Associate Editor}
 
{\bf Thank you for your submission towards TSE. The reviewers have carefully reviewed this paper and given their expertise and request for a major review I have requested the same. The significant feedback they have given is very thorough. Please evaluate the reviewers comments and I very much look forward to receiving your revised submission.}

Thank you for the opportunity to resubmit. Please thank the reviewers-- their comments were insightful and this draft is much improved, thanks for their input.

 \subsection*{Rewiewer1}
 
 
 {\bf This journal paper extends a published paper from the authors in IEEE TSE 2019. In this submission, the authors have used additional SE and non-SE datasets for evaluating DODGE. Authors have also proposed and evaluated the use of intrinsic dimensionality to understand when DODGE can be used.
I have following suggestions for the authors for revising the paper:}


 Thank you for your comments. Please see our comments below (and the associated \revised{BLUE} text in the paper).
 
\subsubsection*{Comment 1.1} {\bf  In Section 3.2, the authors state that "We do not compare against all hyperparameter optimization methods (since any such comparison would take too long to read). Instead, we use hyperparameter optimization methods widely seen in the SE literature". However, this is not a convincing argument since there has been significant amount of research done in the machine learning community on hyperparameter tuning and optimization. For a standard task such as binary classification, we should compare DODGE with more baselines and algorithms. Please see this link for some open-source frameworks: https://medium.com/@sivasai.yadav/10-hyperparameter-optimization-frameworks-8bc87bc8b7e3}

%\citeresp
%\respto
 Great comment! Your comment (and a similar one from Reviewer3) has lead to an amazing new result, which we include in this article.

We read that Medium article with great interest. We checked the algorithms listed there in Google Scholar.
From that, there was a    a truly outstanding candidate for comparison- the HYPEROPT system.  If you search
  Google Scholar         ``Hyper-parameter optimization'' then what you'll see is that the HYPEROPT papers 
 Bergstra et al.~\cite{bergstra2012random,bergstra2011algorithms} have  2159 citations  and 4982 citations each (and the  nearest other work was a 2013 paper by Thornton et al. on Auto-WEKA~\cite{thornton2013auto} with ``only'' 931 citations.). Accordingly,
 when we compare DODGE against an algorithm
 not developed by the SE community, we   used
 the  HYPEROPT(TPE) algorithm that you suggested and which is recommended by 
  Bergstra et al. 
  
  For our experiments,
  we use the TPE implementation from Bergstra's HYPEROPT toolkit~\cite{10.5555/3042817.3042832} (which is one of the tooklits mentioned in https://medium.com/@sivasai.yadav/10-hyperparameter-optimization-frameworks-8bc87bc8b7e3)   {\citeresp{1.1a}} {\citeresp{1.1b}}.
  
Now there's the exciting part: HYPEROPT works {\bf in reverse} to DODGE. If you look at how HYPEROPT compares to DODGE  {\citeresp{1.1c}},
you'll see that where DODGE does best (for low dimensional data) is where HYPEROPT does worse. That is, in a result that underlines the main message of this paper, \begin{quote}{\bf Intrinsic dimensionality can be used to select algorithms that are appropriate for different data sets}.\end{quote}

More generally,   algorithms developed for general AI problems (e.g. TPE) may not be ideal for SE data.  Hence we have added text to the paper  {\citeresp{1.1d}} the suggestion that researchers (a)~take the time to understand how SE data might be {\em different} to data from other domains; then (b)~reflect on how those differences might inform algorithm choice.

And there's an even more exciting part. Looking over the repo for HYPEROPT, we can see an opportunity to   quickly do a pull request where DODGE is added to HYPEROPT. Which means that, as a result of your comment, we can see away to distribute DODGE very broadly in the research community.


We think these new HYPEROPT results and opportunities are an  important and insightful and exciting addition to the prior draft-- and we would not have gone there
without your urging (ditto to Reviewer3). 

So we cannot thank you enough (and Reviewer3) for pushing us into making the comparison of DODGE with other algorithms.


\subsubsection*{Comment 1.2} {\bf New material - The new material in this submission is focused on (a) Evaluation on more datasets, particularly non-SE datasets (b) Usage of dimensionality to evaluate when DODGE will not be applicable.

I am not convinced if the new material is a significant contribution. For instance, authors use the poor performance of DODGE on non-SE datasets to motivate the use of intrinsic dimensionality to evaluate the applicability of DODGE. Also, as per Conjecture 1, authors state that DODGE works well on SE data but fails elsewhere. This actually highlights the gaps in the SE datasets which are used for evaluation of DODGE. It's unclear why authors have not used datasets from recent SE tasks such as code summarization, type inference, etc. which are high dimensional datasets.}

We hear your complaint-- and we agree. Our {\em Future Work} section stresses the need to explore more data sets
{\citeresp{1.2}}

As further evidence that we agree with you, we note that this paper actually does (as you say) ``explore gaps in the datasets what are used to evaluate DODGE?''. Please consider:   the prior version of this paper (IEEE TSE'19) only showed {\em successful}  cases where our method worked.  As you say, that is unsatisfactory. What we did in this paper was:
\begin{itemize}
\item
Expand the space of domains..
\item
... until we found examples where our method did not work...
\item
... then we precisely characterized the reasons why some examples worked and some failed (intrinsic dimensionality).
\end{itemize}
Further, we note that this discovery (of the importance of intrinsic dimensionality) is unique in SE analytics.   
In our view, that is good science and worthy of publication (i.e. using intrinsic dimensionality we can peek at data to select an optimization algorithm,  before running any inference algorithm).

But what is your view?

% As you say, there are many domains we could have explored including (e.g.) code summarization tasks. Now if we were claiming that our method works for all SE analytics, that would be a fatal flaw in this paper. However {\bf that is 
% \underline{absolutely not} our case.}

% What we show here is that the kinds of data seen in  hundreds of prior analytics papers can be divided up according to intrinsic dimensionality {\em AND} we can we can show where our methods succeed and fail.  We hope you'd agree that is a novel and important result. Perhaps, like us,
% you  have to review   dozens of
% papers each year  that propose yet another minor variation on "we applied learnerX to a data set and it worked better
% than learnerY'' {\bf without any explanation of why learnerX might be better than learnerY}.  

% So we think this paper is very
% important.  We offer a unique conclusion that is missing from the general software analytics literature. Specifically:  we can explain why our methods succeed or failure (intrinsic dimensionality). Further, that reason speaks to a core property that distinguishes AI-for-SE from other AI domains. This is useful for many reasons such as (a)~optimizer selection (which can be accomplished before any optimizer is run) and (b)~point \#2 on this list.

% With respect, we  disagree, for three reasons:
% \begin{enumerate}
% \item

% \item
% Now please consider the generality of what we are showing here: standard AI algorithms (HYPEROPT) fail due a previously unreported feature of SE data (that is intrinsically simpler than many of the data set used to develop
% AI algorithms that are widely applied in software analytics\footnote{The reviewer is probably aware than what we call where the ``non-SE'' us the same data used to develop and debug random forests, SVMs, topic modeling, etc etc and all the other learning algorithms used in SE.}).
% Now please consider the impact of that observation:  much prior work could now be revisited and clarified. Certainly in our lab,
% this paper is the basis of years of future research planning where we will explore
% if those  
% clarifications lead to simpler models that are more understandable, and  more audit-able and improvable, by humans.
% \item
% If \#1 and \#2  is  convincing to you, then we offer another argument. Reviewers for the last version of this paper (which appeared in TSE'19) had concerns about the external validity of our conclusions. Before, we only had results from 16 data sets. Now we can demonstrate our effects on dozens and dozens of other data sets. 
% \end{enumerate}

\subsubsection*{Comment 1.3}

{\bf Also, another weakness of the evaluation methodology is that it's only focused on binary classification tasks and non-deep learning methods. These are major limitations in my opinion and would add significant contribution, if addressed.}

We completely  agree and we are looking now at regression and deep learning systems. That analysis has no definitive results (yet) and we are finding so many interesting issues that it looks like each of those areas (regression, deep learning) will require their own paper. Just to give you a sense of those interesting issues we share here some preliminary results about an on-going investigation into issue close time:
\bi
\item
Other authors have proposed the use of state-of-the-art deep learners to explore that issue.
\item When applied to the data we have here, repeated $N$ times for statistical validity, those deep learners need eight years of CPU to terminate. 
\item
On the other hand, we have found that a decades-old perceptron implementation terminates on this data in five hours.
Further, hyperpameter optimization of the decades-old perceptron does better than tuning the state-of-the-art very slow deep learner.
\item
Which is almost like saying a really dumb fast learner is better than a really smart slow learners since the former can be tuned faster.
\ei
Now clearly, we cannot offer that last point as a conclusion
{\em without} extensive further investigation-- at which point it is sounding like something worthy of its own paper rather that an addition to this paper.
 

\subsubsection*{Comment 1.4} {\bf  Writing style - While the paper is generally well written, there are several broad statements which needs to be substantiated with examples and data:

- Pg. 3: "learning good control settings for a learner can take days to weeks to years {...}" - This sounds like an over generalization without showing specific examples or factual data from prior work, the citations provided are not sufficient. Also, looking at the example provided from Lam et. al, it's unclear how and whether they needed weeks of CPU time.}

We agree that that sentence is over-reach. We  have deleted that paragraph.

{\bf - Pg. 3: "CPU facilities must be paid for. Cloud computing environments {...}" - This statement is again too abstract and ignores the widely available cloud computing resources available today at significantly low cost compared to just a few years ago. Even for academia, there are a lot of grants available beyond the university funding which enables researchers to use cloud resources.}

You are quite correct to point that out. We have deleted those specific remarks.


{\bf - Pg. 3: "we note that in our own lab {...}" - It's hard to put things into perspective without more context and details.}

Indeed. We have deleted that remark.

{\bf 4. Minor comment - The abstract assumes that the reader is familiar with DODGE which may not be the case.}

Good point-- we added some extra text to the new abstract
{\citeresp{1.4}}.


\subsection*{Reviewer2}


 Thank you for your comments. Please see our comments below (and the associated \revised{BLUE} text in the paper).
 
{\bf 

Software analytics is a hot topic in SE research, and the problem of hyperparameter optimization is a key problem in software analytics. Thus, this paper is a great fit for TSE. 
Moreover, the finding regarding the limits of DODGE's effectiveness was really interesting. DODGE performs considerably faster than more rigorous approaches, so there is a burning question about whether trading rigor for speed is worth it. The evaluation provides convincing evidence that DODGE is effective for software analytics, and the paper does an excellent job of clarify why DODGE is effective. It also makes it clear when DODGE would likely not be effective---i.e., when the data has high dimensionality.}

~\\

Thank for those words. Much appreciated.

~\\

 {\bf No prior evaluation of DODGE, like the one reported in the paper, has been reported in the literature, and the finding about DODGE's effectiveness with respect to the dimensionality of data is new.
The evaluation study was well conceived and thoroughly reported. A key potential concern about an evaluation like this is the representativeness of the data used to test the approach. In this work, the researchers were very thorough, using a large number of data sets that cover a large number of topics, including ones outside SE. In the end, I was well convinced that the results were not significantly biased based on the data. 
I also commend the authors on their thorough reporting of threats to validity. No empirical study is perfect, and it's important for readers to understand how results may be wrong or misleading. The authors addressed this requirement well, and I didn't notice any significant concerns that were missing from the discussion. The authors were very thorough in their coverage and discussion of relevant prior work, and I didn't notice any important works that were missed.}

~\\

Thank you! You are very kind.
 

\subsubsection*{Comment 2.1}
{\bf The only real issues I had with this paper were regarding its presentation. The presentation was by no means bad--actually, it was pretty good! There were just a couple issues that should be addressed.
The one global concern I had was that the paper is written in such a way that seems to assume that the reader is already familiar with all the concepts covered in the paper. Many concepts are mentioned without ever being introduced. For example, the abstract dives in, talking about "DODGE-ing away", but what DODGE is is never introduced. To a reader not already familiar with DODGE, this sentence would make little sense.}

We agree! Reviewer1 was unhappy about that too. So we have fixed that for this draft
{\citeresp{1.4}}.

\subsubsection*{Comment 2.2}

{\bf That sort of pattern repeats throughout the paper. To address this issue, I suggest that the authors make pass through the paper, trying to place themselves in the shoes of a general SE reader, and identifying everyplace that a new concept is introduced and making sure that some text is present to introduce the concept in case the reader is not already familiar.}

Thank you that timely comment. We agree- this  paper  explores  a  wide  range  of  technologies. Hence,  at that start of this paper,   it  is  appropriate  to  offer  some introductory notes on that material {\citeresp{2.2}}. 

\subsubsection*{Comment 2.3}
{\bf In addition to this global issue, I also spotted the following minor issues with the writing.}

Thank for your 39 detailed editorial improvements. We had implemented them all.
Many thanks for your care and attention
to this review.

As to your other 4 suggestions:
\bi
\item As you correctly pointed out, we needed to expand our needlessly terse headings to section 2,3,4;
\item
Also, at your suggestion, we added a footnote with a short description of the UCI repo-- see Footnote3 on page5.
\ei

\subsection*{Reviewer3}


 Thank you for your comments. Please see our comments below (and the associated \revised{BLUE} text in the paper).
 
{\bf 
This is a very relevant paper for researchers and practitioners who want to use ML models to perform SE tasks.
I am happy to see an experiment with a large number of data sets from many different SE and non-SE domains.
I also liked the general structure of the paper.}

Thank you for those kind words. 

In the following you make many important points and, as you can see, we have made many suggestions in response to your comments (e.g. now we compare DODGE with optimization technology from the general AI literature).
 

\subsection*{Comment 3.1}
 
{\bf My complaint with respect to the proposed experiments is that it is not very clear what DOGE is being compared against. They make the following statements:
“This paper does not compare DODGE against all other learners and all other hyperparameter optimizers (since such a comparison would not fit into a single paper). Instead, we use baselines as found in the SE literature for bad smell detection, predicting Github issue close time, bug report analysis, and defect prediction.”
After reading the introduction and this section, I was expecting to see a clear comparison on the +100 data sets between Dodge and other hyperparameter optimizers,}

You make a good point. Further,
you should know that Reviewer1 had a similar complaint and sent us a list of current hyperparameter optimization frameworks from outside of SE.

Based on your feedback (and that of Reviewer1), we expanded our study-- to great effects. Please see above (Reviewer Comment 1.1).

% Instead, each experiment compares DODGE against specific optimizers or learners or a combination of both, which was very confusion. Sometimes DODGE is better than an optimizer, other times, it is better than a learner, which made it hard to think about what DODGE is. For instance, in Section 3.5.1, I got the impression that DODGE was better than the hyperparameter optimization DE presented in section 3.1 (although it is not clearer whether DODGE and DE used the same learners to produce the results). Then in Section 3.5.3, it looks like the comparison is between DODGE and random forest, and later, in section 3.5.5, it looks like the comparison is again between DODGE and many other learners without optimizations at all.

% In general, I understand the value of the current experiments and what DODGE does. I also understand that it may be hard to make a direct comparison with other optimizers and that there is value in comparing DODGE against the best results presented in previous paper, no matter whether the previous authors used an optimizer or not, since the goal is to understand when DODGE performs well.

% {\bf Instead, each experiment compares DODGE against specific optimizers or learners or a combination of both, which was very confusion. Sometimes DODGE is better than an optimizer, other times, it is better than a learner, which made it hard to think about what DODGE is. For instance, in Section 3.5.1, I got the impression that DODGE was better than the hyperparameter optimization DE presented in section 3.1 (although it is not clearer whether DODGE and DE used the same learners to produce the results). Then in Section 3.5.3, it looks like the comparison is between DODGE and random forest, and later, in section 3.5.5, it looks like the comparison is again between DODGE and many other learners without optimizations at all.

% In general, I understand the value of the current experiments and what DODGE does. I also understand that it may be hard to make a direct comparison with other optimizers and that there is value in comparing DODGE against the best results presented in previous paper, no matter whether the previous authors used an optimizer or not, since the goal is to understand when DODGE performs well.}

\subsubsection*{Comment 3.2}

{\bf The authors need to improve the description of the experiments. I don’t think anyone expects they would have to use all tools in the field. However, just saying that the evaluation would not fit in the paper or it would take too long to read it does not add much. It would be much better to explain why the authors did not compare the presented optimizers and learners in a uniformed way across all the data sets.  I  think  it  could  be  useful  if  the  authors  clarify  the overall  goal  and  design  of  the  experiment  earlier  in  the paper and what are all the learners and hyperparametersthat they used in DODGE. If I understood it correctly, this is fixed and did not change from experiment to experiment(even if the baseline is just random forest or svm)}

You raise an important point. Thank you for that.
We needed to add a rationale for the multiple  performance measures and evaluation rigs used   here {\citeresp{3.2}}.
 
Also, regarding the specific items you mention about (goal, design), we have have made the changes you suggested \citeresp{3.2a} \citeresp{3.2b} \citeresp{3.2c} \citeresp{3.2d}.


~

{\bf 
Another concern that I have with respect to the fact that this is not a direct comparison with other optimizers is whether the existing models were tuned for different metrics, such as precision, accuracy, f-score, instead of the metrics used in this paper. It would be good to have more details about which metrics were used to build these models and what is the impact of it for this evaluation. I understand that different papers can use different metrics, but it feels like comparing one model that was manually tuned for one metric against another tool that was automatically optimized using other metrics can lead to problems. The authors need to clarify whether this was the case.}

You are right-- an apples to apples comparison is important or the reason the  prior draft based all its evaluations on prior work (where we tried to tune for the same goals as they).

But we also take your other point (see commend 3.1)  that {\em it is not enough} just to adopt all the assumptions of prior
work. Hence, in this draft we also compared against a state of the art tool from AI-- which produced some very insightful results.  (See Reviewer Comment 1.1)


  
\subsubsection*{Comment 3.3}
{\bf Another concern that I have with respect to the fact that this is not a direct comparison with other optimizers.  For instance, it is not clear how the authors come up with the parameters for the learners in the non-SE data set. }



Thank you for that comment-- we have added that detail. {\citeresp{3.3}}.
 
 
 Now some of those SOTA studies were
unhappy with those parameters so they did some hyperparameter optimization with genetic algorithms
(see Panichella et al.~\cite{Panichella:2013}). We note that our methods for finding those parameters (with DODGE)
do better than that prior work.

Also,   please consider the new HYPEROPT(TPE) results in this paper  {\citeresp{1.1a}} {\citeresp{1.1b}}  {\citeresp{1.1c}}. Here, we allow two algorithms to explore a wide range of tuning options (TPE and DODGE). So we think this paper has very good
controls on how the hyperparamters are set.

\subsubsection*{Comment 3.4}

{\bf By the way, I do like the false alarm metric, but it would be great if it authors could cite more papers that also used this metric in their experiments to give to the reader a better understand about how spread is this metric in the SE community, compared to standard metrics like precision, accuracy, and f-score.}

   Thanks for the comment. Like you, we have thought long and hard about what are appropriate evaluation metrics for SE. If you look at Figures 21.1 and 23.2 of book {\em Data Science for Software Engineering: Sharing Data and Models}, we list dozens of criteria current seen in the software analytics literature. All these different measures reflect different domain concerns. One reason to depreciate standard machine learners, and turn instead to   multi-objective optimization, is that learners usually have their success criteria hard-wired into their algorithms (while optimizers accept those performance criteria as customizable inputs).   So, in our view, no eval criteria is always ``right'' but some are useful (so we need to pivot to different goals, as domains require it).~\\ Also, for other papers that use false alarm in SE, there are many (e.g.~\cite{10.1145/2938503.2938553,BENER2015453}). As to accuracy and precision, we have written much on how these measures become unreliable when data sets have imblanaced class distributions (please see Menzies et al. 2007 TSE paper~\cite{Menzies:2007prec}). 
  

\subsubsection*{Comment 3.5}

{\bf As I mentioned earlier, I liked the overall structure of the paper, however, some of the terms used in the paper are only defined much later making it hard to read the paper.  It would be very helpful if the authors could improve the description of these terms as soon as they are introduced in the paper. }

You are correct to raise this point. Reviewer2 had similar concerns. To address this point, we have added nearly a page of introductory tutorial material {\citeresp{3.5}}.

\subsubsection*{Comment 3.6}
{\bf Although the paper has a good set of references, I think the authors should improve the references for the papers that use deep learning in the SE field. The current version of the paper gives the impression that there isn’t much research out there on deep learning for SE (and consequently, data sets with high intrinsic dimensionality). }

This is a good point. We have offered some public comments on this matter in this latest draft  {\citeresp{3.6}}.

Also, privately for the reviewers of this paper, we can offer another remark on DL and tuning. Please see our response to reviewer comment 1.3.

\subsubsection*{Comment 3.7}

{\bf Minor comments: typos and other small changes.}

Fixed! Thank you!
 
{\bf Section 3.1 does not list KNN but it looks like it was used in the experiments.}

Wow! Good catch. Fixed now
{\citeresp{3.7}}.
